The Science Case for ALMA Band 2 and Band 2+3

We discuss the science drivers for ALMA Band 2 which spans the frequency range from 67 to 90 GHz. The key science in this frequency range are the study of the deuterated molecules in cold, dense, quiescent gas and the study of redshifted emission from galaxies in CO and other species. However, Band 2 has a range of other applications which are also presented. The science enabled by a single receiver system which would combine ALMA Bands 2 and 3 covering the frequency range 67 to 116 GHz, as well as the possible doubling of the IF bandwidth of ALMA to 16 GHz, are also considered.

==> fig_class0-evol.tex <==
\begin{wrapfigure}{R}{8cm}
  \caption{\footnotesize The correlation of global against source average dust
    temperature. Sources evolve to higher dust temperature as they start to
    heat the circumstellar envelope. \citep{2009A&A...493...89E}.}
\label{fig_class0-evol}
\includegraphics[width=7.5cm]{Figures/class0-evol.png}
\end{wrapfigure}



==> fig_dsp-ratio.tex <==
\begin{wrapfigure}{R}{8cm}
  \caption{\footnotesize The results of a model of deuterium fraction in the
    gas around a young massive star as a function of time since the start of
    heating by the star.  The thin lines show the ratio \ntwodplus\/\ntwohplus
    and while DNC/HNC is shown as thick lines.  The high initial deuteration
    fraction is quenced much more rapidly in \ntwodplus\/\ntwohplus than in
    DNC/HNC. The dotted and dashed curves correspond to different evolutionary
    ages of the gas when the heating starts. \citep{2014MNRAS.440..448F}. }
\label{fig:dsp-ratio}
\includegraphics[width=7.5cm]{Figures/time-dep-dratio.png}
\end{wrapfigure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

